Image Generation for Efficient Neural Network Training in Autonomous Drone Racing

Drone racing is a recreational sport in which the goal is to pass through a sequence of gates in a minimum amount of time while avoiding collisions. In autonomous drone racing, one must accomplish this task by flying fully autonomously in an unknown environment by relying only on computer vision methods for detecting the target gates. Due to the challenges such as background objects and varying lighting conditions, traditional object detection algorithms based on colour or geometry tend to fail. Convolutional neural networks offer impressive advances in computer vision but require an immense amount of data to learn. Collecting this data is a tedious process because the drone has to be flown manually, and the data collected can suffer from sensor failures. In this work, a semi-synthetic dataset generation method is proposed, using a combination of real background images and randomised 3D renders of the gates, to provide a limitless amount of training samples that do not suffer from those drawbacks. Using the detection results, a line-of-sight guidance algorithm is used to cross the gates. In several experimental real-time tests, the proposed framework successfully demonstrates fast and reliable detection and navigation.

==> images/finite_state_machine.tex <==
\begin{tikzpicture}[>=stealth',shorten >=1pt,auto]
   \tikzstyle{state} = [draw, very thick, fill=white, rectangle, minimum
   height=3em, minimum width=7em, node distance=8em]
   \tikzstyle{stateEdgePortion} = [black,thick];
   \tikzstyle{stateEdge} = [stateEdgePortion,->];
   \tikzstyle{edgeLabel} = [pos=0.5, text centered];

   % Position states
   \node[initial,state,accepting, name=landed] {LANDED};
   \node[state, name=takeOff, below of=landed] {TAKE\_OFF};
   \node[state, name=aiming, left of=takeOff, below of=takeOff, xshift=-8em] {AIMING};
   \node[state, name=refining, below of=takeOff] {REFINING};
   \node[state, name=flying, below of=aiming] {FLYING};
   \node[state, name=waiting, below of=refining, yshift=-5em] {WAITING};
   \node[state, name=leaving, below of=flying, yshift=-4em] {LEAVING};
   \node[state, name=crossing, right of=leaving, xshift=16.7em] {CROSSING};
   %\node[state, name=landing, right of=landed] {LANDING};

   % Connect the states
   \draw (landed.south)
      edge[stateEdge] node[edgeLabel, xshift=-6em]{\emph{User input}}
      (takeOff.north);

   \coordinate (aimingNorth) at ($(aiming.north) + (0, 6.5em)$);
   \draw (takeOff.west) edge[stateEdgePortion] node[edgeLabel]{\emph{altitude}
      $\geqslant$ \emph{200cm}} (aimingNorth);
   \draw (aimingNorth) edge[stateEdge] (aiming.north);

   \draw ($(aiming.south) + (-.2em,0)$)
      edge[stateEdge] node[edgeLabel, xshift=-6em]{\emph{window $\ne$ 0}}
      ($(flying.north) + (-.3em,0)$);
   \draw ($(refining.west) + (0,-1em)$)
      edge[stateEdge, bend right=30] node[edgeLabel, text
      width=6em]{\emph{$\neg$ crossing $\land$ window $\ne$ 0}}
      ($(flying.north) + (.5em, 0)$);
   \draw ($(refining.west) + (0, .5em)$)
      edge[stateEdge] node[edgeLabel, yshift=3em, text
      width=6em]{\emph{$\neg$ crossing $\land$ window $=$ 0}}
      ($(aiming.east) + (0, .3em)$);
   \draw ($(flying.south east) + (0, 1em)$)
      edge[stateEdge, bend right=35] node[edgeLabel,
      yshift=-3em]{\emph{t > 13ms}}
      ($(refining.south) + (-.3em, -.1em)$);
   \draw ($(refining.south) + (3em, 0)$)
      edge[stateEdge] node[edgeLabel]{$\neg$ \emph{ready}}
      ($(waiting.north) + (3em, 0)$);
   \draw ($(waiting.north) + (1em, 0)$)
      edge[stateEdge] node[edgeLabel]{\emph{ready}}
      ($(refining.south) + (1em, 0)$);

   \coordinate (refining2ClosedA) at ($(refining.east) + (5.1em, 0)$);
   \draw (refining.east) edge[stateEdgePortion] (refining2ClosedA);
   \draw (refining2ClosedA)
   edge[stateEdge] node[edgeLabel, rotate=-90, xshift=-4em,
   yshift=1em]{\emph{crossing\_condition}}
   (crossing.north);

   \draw (crossing.west)
   edge[stateEdge] node[edgeLabel,
   yshift=-.5em]{\emph{altitude $\geqslant$ MAX\_GATE\_HEIGHT}}
   (leaving.east);

   \coordinate (leaving2ClosedA) at ($(leaving.west) + (-5em, 0)$);
   \coordinate (leaving2ClosedB) at ($(aiming.west) + (-5em, 0)$);
   \draw (leaving.west) edge[stateEdgePortion] (leaving2ClosedA);
   \draw (leaving2ClosedA) edge[stateEdgePortion] node[edgeLabel,
   rotate=90, xshift=5em, yshift=.8em]{\emph{delay > LEAVING\_TIME}} (leaving2ClosedB);
   \draw (leaving2ClosedB) edge[stateEdge] (aiming.west);


   % Draw the velocities
   \node[draw,rectangle,dashed,minimum width=4em,node distance=3cm,right
   of=takeOff, yshift=-3em] (velTakeOff) {$\mathbf{v}=(0,0,.5)$};
   \path[draw,dashed] (takeOff.east) -- (velTakeOff);

   \node[draw,rectangle,dashed,minimum width=4em,node distance=2cm,below
   right of=flying,yshift=-1em] (velFlying) {$\mathbf{v}=\texttt{PID()}$};
   \path[draw,dashed] (flying.south) -- (velFlying);

   \node[draw,rectangle,dashed,minimum width=4em,node distance=2cm,below
   left of=waiting] (velWaiting) {$\mathbf{v}=(0,0,0)$};
   \path[draw,dashed] (waiting.south) -- (velWaiting);

   \node[draw,rectangle,dashed,minimum width=4em,node distance=2cm,above
   left of=leaving,yshift=1em] (velLeaving) {$\mathbf{v}=(.5,0,0)$};
   \path[draw,dashed] (leaving.north) -- (velLeaving);

   \node[draw,rectangle,dashed,minimum width=4em,node distance=2.5cm,above
   right of=crossing] (velCrossing) {$\mathbf{v}=(.5,0,0)$};
   \path[draw,dashed] (crossing.north) -- (velCrossing);

   \node[draw,rectangle,dashed,minimum width=4em,node distance=2cm,above
   left of=aiming] (velAiming) {$\psi=0.05$};
   \path[draw,dashed] (aiming.north) -- (velAiming);
\end{tikzpicture}


==> images/gate_detection_evaluation.tex <==
\begin{tabular}{|r|l|}
	\hline
	AP (IoU=0.5) & 0.906 \\
	AP (IoU-0.75) & 0.633 \\
	\hline
\end{tabular}


==> images/system_diagram.tex <==
\begin{tikzpicture}[node distance=2cm,-latex]

\pgfdeclarelayer{background}
\pgfdeclarelayer{foreground}
\pgfsetlayers{background,main,foreground}
\tikzstyle{sensor}=[node distance=1.5cm,draw, rectangle,fill=blue!20, text
width=2cm,text centered,minimum width=2cm, minimum height=1cm]
\tikzstyle{perc}=[draw, node distance=4cm,draw, rectangle,fill=green!20, text
width=2cm,text centered,minimum width=2cm, minimum height=1cm]
\tikzstyle{control}=[draw, node distance=3cm,draw, rectangle,fill=red!20,
text width=2.5cm,text centered,minimum width=.5cm, minimum height=3cm]

%% Sensors Nodes 
\node[sensor] (cam) {Camera};
\node[sensor,below of=cam] (vicon) {Motion capture};
\node[sensor,below of=vicon] (lidar) {Lidar};
\node[node distance=1cm,above= of cam.west,anchor=west] (sensors) {Sensors};

\begin{pgfonlayer}{background}
    \node[fit=(sensors) (cam) (vicon) (lidar), draw,fill=yellow!20] (frame) {}; 
\end{pgfonlayer}

%% Perception Nodes
\node[perc,node distance=4cm,right of=cam] (cnn) {CNN};
\node[perc,right of=cnn, xshift=2em] (median) {Median Filter};
\node[node distance=1cm,above= of cnn.west,anchor=west] (perception) {Perception};

\begin{pgfonlayer}{background}
    \node[fit=(perception) (cnn) (median), draw,fill=yellow!20] (frame) {}; 
\end{pgfonlayer}

%% Control Nodes
\node[control,node distance=6cm, minimum width=2cm,below of=cnn] (state)
    {State Machine};
\node[control,right of=state,minimum width=0.5cm,minimum
    height=1cm,yshift=1cm,xshift=-.5cm,text width=1cm]
    (pid) {PID};
\node[control,right of=pid,minimum width=2cm,minimum height=1cm, xshift=2cm]
    (safety) {Safety Mechanism};
\node[control, node distance=2cm,below of=pid,minimum width=2cm,minimum
    height=1cm,yshift=-1.5em,xshift=1.5em] (low) {Low Level Control};
\node[node distance=2cm,above= of state.west,anchor=west] (controller)
    {Control};

\begin{pgfonlayer}{background}
    \node[fit=(state) (pid) (safety) (low) (controller), draw,fill=yellow!20]
        (frame) {}; 
\end{pgfonlayer}

%% Connections
\draw[thick] (cam) -- node[yshift=1em]{\emph{image}} (cnn);
\draw[thick] (cnn) -- node[yshift=1em]{\emph{prediction}} (median);
\draw[thick] (lidar.east) -- node[yshift=-3em,
    xshift=-0.5em]{\emph{height}} ++(1cm,0) |- (state);
\draw[thick] ($(vicon.south east)!0.33!(vicon.north east)$) -| node[yshift=-5.0em,
    xshift=-1.5em]{\emph{pose}} ($(pid.north west)!0.33!(pid.north east)$);
\draw[thick] ($(vicon.north east)!0.33!(vicon.south east)$) -| node[yshift=-6.0em,
    xshift=1.5em]{\emph{pose}}(safety.north);
%\draw[thick] (pid.west) -- ($(state.north east)!0.17!(state.south east)$);
\draw[thick] (state.east) -|
    node[xshift=-9em, yshift=-1em]{\emph{velocity command}}
    ($(safety.south west)!0.33!(safety.south east)$);
\draw[thick] (pid) -- node[text width=2cm,yshift=.5cm]{\emph{velocity command}} (safety);
\draw[thick] ($(safety.south west)!0.66!(safety.south east)$) |-
    node[xshift=-3em,yshift=-1em]{\emph{velocity command}}
    (low.east);
\draw[thick] ($(median.south east)!0.33!(median.south west)$) --
    node[xshift=-2em, yshift=-3.5em]{\emph{filtered prediction}} ++(0,-2cm)
    -|($(pid.north west)!0.68!(pid.north east)$);
\draw[thick] ($(median.south west)!0.33!(median.south east)$) -- ++(0,-.5cm) -|
    node[xshift=-2em, yshift=-4.5em, text width=2cm]{\emph{filtered prediction}}
    ($(state.north west)!0.68!(state.north east)$);
\end{tikzpicture}


==> sections/detection_results.tex <==
\begin{table}[!b]
  \centering
  \caption{Average precision and recall for different IoU
  thresholds.}
  \begin{tabular}{r|l|l|l|l}
      IoU threshold & \multicolumn{2}{c|}{Semi-synthetic} & \multicolumn{2}{c}{Real} \\
      %\hline
                    & AP & AR & AP & AR \\
      \hline
      0.50 & 0.891 & 0.647 & \textbf{0.905} & 0.576\\
      0.75 & \textbf{0.797} & 0.601 & 0.648 & 0.471\\
      0.90 & \textbf{0.436} & 0.396 & 0.011 & 0.050\\
  \end{tabular}
  \label{tab:detection}
\end{table}

\begin{table}[!b]
  \centering
  \caption{Average precision for different IoU
    thresholds and for every class. (synthetic dataset only)}
  \begin{tabular}{r|l|l|l}
    Class & AP$_{0.5}$ & AP$_{0.75}$ & AP$_{0.9}$\\
      \hline
      Target gate & 0.891 & 0.797 & 0.436 \\
      Forward gate & 0.819 & 0.726 & 0.231\\
      Backward gate & 0.907 & 0.811 & 0.382\\
      \hline
      mAP & 0.872 & 0.778 & 0.35\\
  \end{tabular}
  \label{tab:detection-detailed}
\end{table}


